A software-defined architecture for control of IoT Cyberphysical Systems

Based on software-defined principles, we propose a holistic architecture for Cyberphysical Systems (CPS) and Internet of Things (IoT) applications, and highlight the merits pertaining to scalability, flexibility, robustness, interoperability, and cyber security. Our design especially capitalizes on the computational units possessed by smart agents, which may be utilized for decentralized control and in-network data processing. We characterize the data flow, communication flow, and control flow that assimilate a set of components such as sensors, actuators, controllers, and coordinators in a systemic programmable fashion. We specifically aim for distributed and decentralized decision-making by spreading the control over several hierarchical layers. In addition, we propose a middleware layer to encapsulate units and services for time-critical operations in highly dynamic environments. We further enlist a multitude of vulnerabilities to cyberattacks, and integrate software-defined solutions for enabling resilience, detection, and recovery. In this purview, several controllers cooperate to identify and respond to security threats and abnormal situations in a self-adjusting manner. Last, we illustrate numerical simulations in support of the virtues of a software-defined design for CPS and IoT.

==> attackmodels.tex <==

\section {Attack Models}
\label {sec:Attackmodels}
The attacks in the network are growing day by day. Tools for scanning, launching, information gathering and  detecting attacks  are also increasing accordingly. A new security architecture is much needed to accommodate all of these attacks. Thus, at first, we should explore and analyze the ways for these attacks which are trying to use to compromise the system \cite{3}. 
\begin{itemize}
	\item \textbf{Trojans:} This type of attack is downloaded on the computer systems as a program file from several resources like the Internet. It aims to break the  network by executing unwanted actions. When the victim host tries to open this file then the system will be injected by this type of attack. There are many types of this attack: Sending Trojans, Remote access Trojans, Proxy Trojans, DoS Trojans and many others.    
	\item \textbf{DoS/DDoS attack:} This type of attack tries to prevent the system's users from accessing the system resources and makes all the resources unavailable for them. However, the Distributed Denial of Services Attack (DDoS)  attempts  to compromise and make the system resources for one or several systems unavailable.
	  
	\item \textbf{Packet Forging attack:} It is also known as "packet injection". This works as a man in the middle attack to interrupt the communication connection by constructing some packets which look like normal ones. There are several tools that the attacker can use to generate a traffic; Tcpinject and Packeth tools.
	
	\item \textbf{Fingerprinting attack:} It is used to identify the network status and to analyze the traffic.  The attackers  try to eavesdrop on the conversation even if it is encrypted by stealing some critical features of the sender and receiver to make disastrous actions. 
	
	\item \textbf{Application Layer attack:}  The detection process of these attacks is much harder than the attacks on the network layer because it uses legitimate connection to smash the web server. This type is classified into four types: the first one  uses the HTTP protocol requests to overwhelm a site, the second one is threaten the SMTP protocol, the third one which related to the FTP protocol and the last one is the SNMP attacks which try to monitor the system after reconfiguration it.       
	
	
	\item \textbf{User attacks:} In this type of attack, the attacker try to gain the supervisor's privilege by working as a legitimate user, or he exploits the vulnerabilities of the local machine and then creates an account inside it. There are different forms of this attack, U2R and R2L are two examples.  
	
	
\end{itemize} 
There are several points which the attacker can inject the system, thus we need to take it in our considerations when designing the model:

\begin{enumerate}
	\item \textbf{Sensor-related attacks:} The attacker may try to listen to the sensed information from the sensor to compromise the system. 
	\item \textbf{Actuator-related attacks:} The attacker tries to compromise the actuator to change the control commands to serve his needs.  
	\item \textbf{Controller-related attacks:} Since all the control and management operations are handled and done by the controller, then compromise this unit consider the main target for him. Securing the controller requires to secure all the underlying unites even the sensors.
	\item \textbf{Communication-related attacks:} Communication channels are also one of the targets of the attacker. Securing these channels is considered one of the most important mechanisms to save the system.   
	
\end{enumerate}	
